Dust Formation in Common Envelope Binary Interaction -- I: 3D Simulations Using the Bowen Approximation

We carried out 3D smoothed particle hydrodynamics simulations of the common envelope binary interaction using the approximation of Bowen to calculate the dust opacity in order to investigate the resulting dust-driven accelerations. We have simulated two types of binary star: a 1.7 and a 3.7 $M_{\odot}$ thermally-pulsating, asymptotic giant branch stars with a 0.6 $M_{\odot}$ companion. We carried out simulations using both an ideal gas and a tabulated equations of state, with the latter considering the recombination energy of the envelope. We found that the dust-driven wind leads to a relatively small increase in the unbound gas, with the effect being smaller for the tabulated equation of state simulations and for the more massive primary. Dust acceleration does contribute to envelope expansion with only a slightly elongated morphology, if we believe the results from the tabulated equation of state as more reliable. The Bowen opacities in the outer envelopes of the two models, at late times, are large enough that the photosphere of the post-inspiral object is about ten times larger compared to the same without accounting for the dust opacities. As such, the prediction of the appearance of the transient would change substantially if dust is included.

==> conclusions/conclusions.tex <==
\section{conclusions}

